Learning Versatile Skills with Curriculum Masking

Masked prediction has emerged as a promising pretraining paradigm in offline reinforcement learning (RL) due to its versatile masking schemes, enabling flexible inference across various downstream tasks with a unified model. Despite the versatility of masked prediction, it remains unclear how to balance the learning of skills at different levels of complexity. To address this, we propose CurrMask, a curriculum masking pretraining paradigm for sequential decision making. Motivated by how humans learn by organizing knowledge in a curriculum, CurrMask adjusts its masking scheme during pretraining for learning versatile skills. Through extensive experiments, we show that CurrMask exhibits superior zero-shot performance on skill prompting tasks, goal-conditioned planning tasks, and competitive finetuning performance on offline RL tasks. Additionally, our analysis of training dynamics reveals that CurrMask gradually acquires skills of varying complexity by dynamically adjusting its masking scheme.

==> fig/attention_goal_jaco.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/raw/attention/attention_all_jaco_goal.pdf}
    \caption{Attention maps (goal-conditioned planning on Jaco).}
    \label{fig:attention_goal_jaco}
\end{figure}

==> fig/attention_goal_quadruped.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/raw/attention/attention_all_quadruped_goal.pdf}
    \caption{Attention maps (goal-conditioned planning on quadruped).}
    \label{fig:attention_goal_quadruped}
\end{figure}

==> fig/attention_goal_walker.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/raw/attention/attention_all_walker_goal.pdf}
    \caption{Attention maps (goal-conditioned planning on Walker).}
    \label{fig:attention_goal_walker}
\end{figure}

==> fig/attention_prompt_jaco.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/raw/attention/attention_all_jaco_prompt.pdf}
    \caption{Attention maps (skill prompting on Jaco).}
    \label{fig:attention_prompt_jaco}
\end{figure}

==> fig/attention_prompt_quadruped.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/raw/attention/attention_all_quadruped_prompt.pdf}
    \caption{Attention maps (skill prompting on quadruped).}
    \label{fig:attention_prompt_quadruped}
\end{figure}

==> fig/attention_prompt_walker.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{fig/raw/attention/attention_all_walker_prompt.pdf}
    \caption{Attention maps (skill prompting on Walker).}
    \label{fig:attention_prompt_walker}
\end{figure}

==> fig/curriculum_trend.tex <==

\begin{figure}[b]
         \vspace{-25pt}
         \centering
         \includegraphics[width=\linewidth]{fig/raw/curriculum/curriculum_walker.pdf}
         \caption{Impact of masking curricula (walker run)}
        %\label{fig:curriculum_trend}
        \vspace{-30pt}
\end{figure}


==> fig/fix_block.tex <==

\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{fig/raw/prompt/prompt_fixed.pdf}
\caption{\textbf{Impact of block-wise masking.}}
%\label{fig:fix_block}
\end{figure}

==> fig/illustration.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,height=0.3\linewidth]{example-image-a}
    \caption{Curriculum masking forms a learning curriculum over skills? (skills learned over time, comparing random and curriculum-based).
    Similar to Figure 3 of Preference Transformer?}
    \label{fig:illustration}
\end{figure}

==> fig/skill.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/raw/prompt/prompt.pdf}
%     \caption{
%     \textbf{Skill prompting results.}
%     We report the zero-shot performance of models pretrained with different masking schemes.
%     Results are averaged over 5 random seeds.
%     % \zhihui{Forecast length is 120.}
%     \zhihui{Table?}
%     }
%     \label{fig:skill}
% \end{figure}

% \begin{table*}[t]
%     \centering
%     
%     \begin{tabular}{l|lll|llll}
% \thickhline
% reward $\uparrow$ & run                                         & stand                                        & walk                                        & reach-bl                                    & reach-br                                    & reach-tl                                    & reach-tr                                    \\ \hline
% Random            & 30.4\scriptsize $\pm$0.9 & 105.1{\scriptsize $\pm$3.4} & 58.7{\scriptsize $\pm$4.0} & 64.3{\scriptsize $\pm$5.5} & 63.1{\scriptsize $\pm$4.2} & 62.4{\scriptsize $\pm$4.3} & 67.4{\scriptsize $\pm$3.9} \\
% Mixed             & 30.6{\scriptsize $\pm$1.4} & 110.4{\scriptsize $\pm$3.3} & 50.9{\scriptsize $\pm$2.2} & 70.4{\scriptsize $\pm$7.6} & 64.8{\scriptsize $\pm$3.7} & 65.8{\scriptsize $\pm$3.9} & 68.9{\scriptsize $\pm$5.3} \\
% Mixed-inv         & 24.6{\scriptsize $\pm$1.3} & 105.5{\scriptsize $\pm$5.0} & 55.3{\scriptsize $\pm$3.1} & 59.8{\scriptsize $\pm$3.3} & 57.2{\scriptsize $\pm$2.7} & 62.8{\scriptsize $\pm$2.1} & 62.7{\scriptsize $\pm$2.8} \\
% Mixed-prog        & 27.0{\scriptsize $\pm$0.5} & 105.2{\scriptsize $\pm$3.7} & 52.8{\scriptsize $\pm$4.8} & 86.8{\scriptsize $\pm$6.4} & 87.7{\scriptsize $\pm$5.1} & 87.9{\scriptsize $\pm$4.8} & 89.2{\scriptsize $\pm$3.8} \\
% CurrMask          & 37.1{\scriptsize $\pm$1.4} & 109.7{\scriptsize $\pm$3.3} & 90.6{\scriptsize $\pm$2.4} & 81.7{\scriptsize $\pm$7.4} & 84.5{\scriptsize $\pm$2.9} & 78.7{\scriptsize $\pm$6.1} & 83.5{\scriptsize $\pm$3.7}
%  \\
% \thickhline
% \end{tabular}
% \caption{\textbf{Skill prompting results.}
%     We report the zero-shot performance of models pretrained with different masking schemes.
%     Results are averaged over 5 random seeds.}
%     \label{tab:skill}
% \end{table*}

% \vspace{-10pt}


==> fig/skill_visualization.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{fig/raw/demo.pdf}
    \caption{Skill prompting visualization.}
    \label{fig:skill_visualize}
\end{figure}
